Can Cooling and Heating Functions be Modeled with Homogeneous Radiation Fields?

Cooling and heating functions describe how radiative processes impact the thermal state of a gas as a function of its temperature and other physical properties. In a most general case the functions depend on the detailed distributions of ionic species and on the radiation spectrum. Hence, these functions may vary on a very wide range of spatial and temporal scales. In this paper, we explore cooling and heating functions between $5\leq z \leq10$ in simulated galaxies from the Cosmic Reionization On Computers (CROC) project. We compare three functions. First, the actual cooling and heating rates of hydrodynamic cells as a function of cell temperature. Second, the median cooling and heating functions computed using median interstellar medium (ISM) properties (median ISM). Last, the median of the cooling and heating functions of all gas cells (instantaneous). We find that the median ISM and instantaneous approaches to finding a median cooling and heating function give identical results within the spread due to cell-to-cell variation. However, the actual cooling (heating) rates experienced by the gas at different temperatures in the simulations do not correspond to either summarized cooling (heating) functions. In other words, the thermodynamics of the gas in the simulations cannot be described by a single set of a cooling plus a heating function with a spatially constant radiation field that could be computed with common tools, such as Cloudy.

==> lit_review_notes.tex <==
\subsection{From papers that cite Gnedin and Hollon} \ca{Treat these as papers to cite in your previous paragraphs.}

https://ui.adsabs.harvard.edu/abs/2012ApJS..202...13G/abstract
\begin{itemize}
    \item Prochaska+13: This paper looks at Hi Lyα absorption to trace high redshift (z=2) IGM (intergalactic medium) properties. Feedback processes impact galaxy formation and properties of the IGM.  Gnedin+Hollon explore this with ART.
    \item De Rijcke+13: This paper calculates composition-dependent radiative cooling and heating curves, aiming to improve upon previous efforts (including Gnedin+Hollon).  Gnedin and Hollon mainly incorporate the radiation field through four well-chosen normalized photoionization rates, Taylor expand the curves to quadratic terms in metallicity, and have an approximation to the cooling and heating curves.  Good to about 10 percent, but can be as bad as a factor of 6.
    \item Vogelsberger+13: Galaxy formation in AREPO code paper.  Use Gnedin and Hollon to show background radiation is important in cooling rate calculations because background radiation affects the thermal state and the ionization state of plasma (the IGM) (also can cite  Efstathiou 1992).  Note, many galaxy formation simulations might use cooling rates that assume collisional ionization equilibrium and exclude background radiation.
    \item Kannan+14:  Galaxy formation with local photoionization feedback from young and old stellar populations, finding that local photoionization is likely an important physical process.  Cites Gnedin and Hollon for incident radiation fields as a cause for slowing gas infall (also Cantalupo 2010). Describe the Gnedin and Hollon model as a general model for cooling in the presence of a radiation field near a galaxy with both stars and AGN. Showed that the spectral behavior of the incident radiation field is mostly dependent on the photoionization rates of a few coolants.  NOTE: This paper and Cantalupo 2010 have similar goals as the Gnedin and Hollon paper.
    \item Ceverino+14: Looks at galaxy formation in low mass high redshift halos with photoionization and photoheating.  Cite Gnedin and Hollon as example of how local photoionization reduces the HI peak of cooling curve, which then reduces cooling for gas in the 1e4-1e4.5K range.  
    \item {\bf  Include in Methods for this paper}  Gnedin 2014:  CROC I paper, cites Gnedin and Hollon to summarize the methods for computing the metallicity-dependent part of cooling and heating functions in non-homogeneous radiation fields.  In the regime of strong radiation fields, the temperature of local thermal equilibrium plasma  depends on the radiation spectrum.
    \item Gnedin and Draine 2014: Implement an empirical model of line overlap in the Lyman and Werner bands, which enhances molecular hydrogen self-shielding in low metallicity ($<10$\%$Z_\odot$) environments, but impact is subdominant to stellar feedback.  Cites Gnedin and Hollon as a more physically realistic model of cooling and heating functions to use.
    \item Feldmann and Mayer 2015:  Argo simulation of a massive galaxy at $z>2$.  Cites Gnedin and Hollon as an example of how photoionization and Compton heating from AGN  reduces cooling
    \item Nick's Notes - {\bf SUPER USEFUL}, summarizes the Gnedin and Hollon paper and discusses the main problem with their approximations (the "catastrophic failures":\\ https://arxiv.org/pdf/1412.5184.pdf
    \item Notes from Klessen and Glover: cites the Gnedin and Hollon paper as an example of accounting for non-equilibrium effects by solving for the non-equilibrium ionization state of the main elements that contribute to high temperature cooling (in the IGM) assuming that the ionization state is dominated by photoionization rather than collisional ionization. \\ https://ui.adsabs.harvard.edu/abs/2016SAAS...43...85K/abstract
    \item McKinnon+16: Cites Gnedin and Hollon as one of three papers to explore how dust impacts cooling rates calculated from local ionizing radiation (also Cantalupo 2010; Kannan+14)
    \item Kannan+16: AREPO implementation of cooling functions that account for the radiation field due to X-rays from stellar binaries (not important) and the hot halo gas (more important).  Also describes Gnedin and Hollon paper as a general model to calculate cooling in the presence of a local radiation field due to stars and AGN).  Radiation fields were found to alter cooling rates of gas near massive O stars and luminous quasars. BUT the quasar mode of feedback Vogelsberger+13 implemented was much less effective than the radio mode. 
    \item 
\end{itemize}

% Significant radiation fields in galaxy formation (EoR), how simulations account for this

% Note:  Useful summary lecture on heating/cooling: http://www.astro.yale.edu/vdbosch/astro610_lecture15.pdf

%  Impact of cooling functions on galaxy formation (mainly gas behavior, star formation, etc)
% \begin{itemize}
   % \item The dynamics of the gas in a galaxy-formation region are governed by hydrostatic equilibrium: gravity trying to compress the gas versus thermal pressure resisting this compression. Thus, the physics of the gas (on both smaller and larger scales) are very sensitive to both the temperature of the gas and the rate of change of the temperature, which is governed by the heating and cooling functions of the gas (\citet{Kannan_2014}). \ca{Last sentence is useful, could use rewording for shorter concise sentences.  First paragraph should start with a more general statement, e.g. "Physical processes in galaxy formation depend on the interplay between cooling and heating processes."}
   % \item \citet{Kannan_2014} provides examples of relevant effects on star formation in a galactic disk, such as that the cooling function of a galactic disk can affect the accretion rate of new material onto the disk, which in turn affects star formation. \ca{These could feed into, "For example, the cooling function of gas in a galactic disc affects..... CITE KANNAN."}
% \end{itemize}
In general, it is clear that the presence of radiation fields will modify the heating and cooling functions of gas.  This happens because the radiation field modifies the abundances of atoms and molecules in various energy and ionization states, and introduces ionizing photons that can increase the energy of the gas.  For each chemical species in the gas, both its photoionization rate and heating rate are set by the radiation field in the environment of the gas \citep{Kannan_2014}.  In other words, both the temperature of the gas and its ionization will be affected by the radiation \citep{Vogelsberger_2013}. 
\ng{The choice of reference is a bit strange here, I am sure CHF were introduced well before Kannan 2014; also, please do not tinker the style even if you do not like it, the editor will be unhappy with all the extra work they will need to undo your tinkering.}

Moreover, there is feedback between the radiation fields and the gas: when the gas absorbs radiation, it will cool by emitting radiation, which contributes to the radiation field \citep{Kannan_2014}.  The radiation field in a galaxy can then be separated into two distinct components: `direct' radiation from light-producing source such as stars, active galactic nuclei, and the cosmic microwave background (CMB), which can be attenuated by intervening matter; and `diffuse' radiation that is emitted by the galactic gas \citep{Cantalupo_2010}.\ng{it is also attenuated by gas}  These two components are not independent of each other, since the diffuse emission from the gas is a response to the direct external radiation field. 
% Radiation fields impact cooling functions (how and citations)
% General discussion of how radiation sources and sinks impact cooling functions, see Kannan 2014 and Cantalupo 2010) 
% \ca{All of this information is good information to include.  I would say, put into full paragraph forms first, and we can cut text later (easier to cut).}
%\begin{itemize}
    %\item In general, the presence of a radiation field will change the abundances of atoms and molecules in various energy and ionization states, and ionizing photons increase the energy of the gas (the freed electrons can gain kinetic energy from the ionizing photons) \citet{Kannan_2014}. 
    %\item For each chemical species in the gas, the radiation field determines both its photoionization rate and its heating rate.
    %\item Radiation fields can both heat gas and decrease the cooling function of the gas, so that the gas cools more slowly \citet{Kannan_2014}.  
    %\item Moreover, there is a feedback between the radiation field and the gas: when radiation is absorbed by gas molecules, that affects the cooling function of the gas, and, as the gas cools, it emits radiation that contributes to the radiation field of the galaxy \citet{Kannan_2014}.
    %\item The radiation field can be separated into two distinct components: 'direct' radiation from light-producing sources (e.g. stars, AGN, the CMB), which may be attenuated by intervening matter; and 'diffuse' radiation emitted by the gas itself \citet{Cantalupo_2010}. These two components are not independent of each other.  
%\end{itemize}

% JUSTIFY WHY THE TOPIC IS INTERESTING AND IMPORTANT - cosmic ray things less important for high z galaxies, mostly in gamma ray regime
%There are predictions and approximations we make for galaxies in cooling functions.  And we want to know if those approximations are valid in high redshifts \ca{during the epoch of reionization}. \ca{Also, in crafting this paragraph, you can go from Cantalupo, to Gnedin and Hollon, to Kannan.} 
%\begin{itemize}
    %\item \citep{gnedin_hollon} demonstrates that the impact of radiation fields on cooling function as depending on a small number (4 or 5) parameters constructed from photoionization rates of specific isotopes, assuming that the gas is optically thin and the radiation field is weak enough that only single-scattering events matter.
    %\item While this approximation scheme produces small median errors (10\%), it can produce catastrophic errors (factor of 2 or greater in 0.1\% of their test cases).
    %\item It is not obvious, a priori, the extent to which these approximations are valid for the regime of reionizing galaxies.
    %\item Shortcomings in models of radiation fields and cooling functions: catastrophic errors, mostly in non-realistic cases %\citep{gnedin2014modeling}; coupling and feedback between gas cooling and the radiation field \citep{Kannan_2014}; assumption that gas is optically thin made by \citep{gnedin_hollon} and \citep{Kannan_2014}, which may fail to be true for a reionizing galaxy.  
%\end{itemize}

% Talk about specific sources of different components of radiation field.
Radiation fields contain contributions from a variety of sources, both local and external to the region of interest.  A radiation field model has to take into account the relative importance of these sources. Work has been done to model the interstellar radiation field of the Milky Way galaxy (e.g. \citet{porter2005new}, \citet{Popescu_2017}), across a wide range of wavelengths \ng{Here you will be torn apart with this choice of references. - need harding, Draine, Matthews(?)}.  From such studies, we can construct a partial list of important sources that make up radiation fields at the present epoch.  These provide useful context for considering radiation fields during much earlier epochs, such as the epoch of reionization. 
At the present epoch, important local contribution to the radiation field include O stars and active galactic nuclei (AGN) which are part of the galaxy under consideration.  These sources produce high energy photons capable of ionizing neutral hydrogen in the ground state.  Older and cooler local stars still contribute to the radiation field, but have a smaller impact on heating and cooling functions because they produce much less ionizing radiation \citep{Kannan_2014}.  Another vital local component of the radiation field comes from re-emission of incident radiation by galactic dust.  This re-emission occurs at infrared and sub-millimeter wavelengths \citep{Popescu_2017}.  This re-emission has direct relevance to the cooling function, as discussed above. \ng{I don't think this is true.} 
The external part of the radiation field at the present epoch includes gamma rays emitted via interactions between cosmic rays and interstellar gas \citep{Popescu_2017, Porter_2017}.  There is also a diffuse background of UV and X-ray photons due to AGN and stars outside of the region of interest.  This contribution is modeled in \citet{Haardt_2012} and  \citet{Faucher_Gigu_re_2009}, updated in \citet{Faucher_Gigu_re_2020}, among others.  
Simulations of gas dynamics in galaxy formation need to take into account the heating and cooling functions of the gas.  Some simulations have incorporated this using the assumption of collisional ionization equilibrium, which ignores the effect of radiation fields on the cooling and heating functions \citet{Vogelsberger_2013} \ng{Need way more refs here.}.  In order to be fully self-consistent, the impact of the radiation field on cooling and heating must be included.  \\
Exact calculation of cooling (or heating) function of gas in the presence of a radiation field is computationally difficult, since it requires radiative transfer calculations \citep{Cantalupo_2010}. However, approximation schemes for the impact of radiation fields on the cooling function have been developed for some regimes. \ng{the following is incorrect, needs revision} Assuming the gas metallicity is close to the solar metallicity $Z_\odot$, \citet{gnedin_hollon} expand the heating and cooling functions in a Taylor series in metallicity.  In the weak radiation field regime, and assuming the gas metallicity is close to the solar metallicity $Z_\odot$, \citet{gnedin_hollon} find that the heating and cooling functions can be approximated by a 3-term Taylor series in metallicity, where the coefficients depend on the radiation field only through 3 parameters constructed from 4 photoionization rates.  The heating and cooling functions are computed using the radiative transfer code \texttt{Cloudy} for a table of ~4000 values of these parameters, as well as temperature and gas density, and linear interpolation in each parameter is used for intermediate values.  This approximation scheme is discussed in much more detail below. \dr{add discussion of where approximation breaks down from this and Nick's notes.} \\
\citet{Cantalupo_2010} combines Adaptive Mesh Refinement (AMR) code with Monte Carlo techniques in order to only do computationally intensive radiative transfer calculations where they are most necessary.    \citet{Kannan_2014} assumes the gas is optically thin, so that the radiation field decreases as $r^{-2}$ from its sources.  Then, computational methods used to model gravity (which also scales as $r^{-2}$) can be utilized to study the radiation field.  By simplifying the chemical evolution of the gas to only two variables, \citet{De_Rijcke_2013} reduces the cooling and heating functions to dependence on only 5 parameters: two parameters to trace the chemical evolution, temperature, gas density, and redshift.  Redshift is needed in this model to determine the background of ultraviolet radiation discussed above.  \citet{Oppenheimer_2013} tracks the ionization states of 11 elements exposed to the extra-galactic background radiation of \citet{Haardt_2012}, assuming the gas is optically thin. \ng{original references needed here} \\
In order to derive these kinds of approximations, these papers assume some functional form of the radiation field, i.e. the intensity as a function of frequency or wavelength.  This is equivalent to choosing both which types of sources to include and an approximate model for the radiation fields from those sources \citep{Kannan_2014, Cantalupo_2010, gnedin_hollon, De_Rijcke_2013, Oppenheimer_2013}.    


%\ca{This should be brief, I think - saying that there are different contributors to the radiation field, some local and some external, and a model should account for the relative importance.  Then, list the possible sources with some commentary. }
%\begin{itemize}
    %\item Work has been done to model the interstellar radiation field of the Milky Way galaxy (e.g. \citep{porter2005new}, \citep{Popescu_2017}), across a wide range of wavelengths.  
    %\item From such studies, we can construct an (at least partial) list of important sources that make up radiation fields at the present epoch.  These provide useful context for thinking about radiation fields at much higher redshift, especially in regarding how these components were different at much earlier times.
    %\item Background radiation (e.g. the CMB): A blackbody spectrum.  Note that the temperature, and therefore frequency peak, of the CMB spectrum will be higher for high-redshift galaxies.
    %\item Cosmic rays: The gamma ray portion of the interstellar radiation field is dominated by emission from cosmic rays interacting with interstellar gas (\citep{Popescu_2017}).
    %\item O-stars and active galactic nuclei produce higher energy photons capable of ionizing neutral, ground state hydrogen.  While older and cooler stars also contribute to the radiation fields, but produce much less ionizing radiation, so have less impact on cooling functions \citep{Kannan_2014}.
    %\item Dust re-emission: When dust grains absorb interstellar radiation, it is later re-emitted at infrared or sub-millimeter (submm) wavelengths (\citep{Popescu_2017}).  Note that this has direct relevance to cooling and heating functions. 
    %\item UV and X-ray diffuse background due to AGN and stars.  Note that this refers to stars and AGN outside the region of interest (\citep{Haardt_2012}).
%\end{itemize}

%Discussion section:  Impact of CMB in Gnedin and Hollon paper?  Does the importance of this component get bigger? 

%Bullet points from introductions to various radiation fields paper. \ca{I think, because these are a bit more local and gamma ray focused, this can be brief.  }
%\subsection{\citep{porter2005new}}
%\begin{itemize}
    %\item High energy gamma ($\gamma$) rays in the Milky way can be generated by inverse Compton scattering of electron cosmic rays with photons in the interstellar radiation field.
    %\item Detailed 3-D spatial information about this radiation field is necessary for $\gamma$-ray calculations.
%\end{itemize}

%\subsection{\citet{Porter_2017}}
%\begin{itemize}
    %\item Gamma ray observations are dominated by signals from cosmic rays interacting with the interstellar radiation field.
    %\item Gamma rays up to ~30TeV experience negligible absorption by the interstellar medium, so these signals are a sensitive probe of cosmic rays over much larger distances than direct detections of cosmic ray particles.
    %\item While the general shape of the gamma ray emission profile of local interstellar space can be reproduced by interstellar emission models, the residuals with observations suggest other effects may be present for the highest energy gamma rays.
%\end{itemize}

%\subsection{\citet{Popescu_2017}}
%\begin{itemize}
    %\item Outside of the solar system, cosmic rays can only be detected via $\gamma$-ray emission via the inverse Compton effect or pion decay.
    %\item To model galactic cosmic rays through $\gamma$-ray observations, we need detailed knowledge of the interstellar radiation field, particularly the mid and far infrared and submillimeter components due to dust emission.
    %\item The presence of dust makes the interstellar radiation field of the Milky Way very difficult to measure, as the radiation fields of stellar sources cannot be directly observed.
    %\item Re-emission by dust in the infrared and submm depends strongly on the initial radiation field, so can place observational constraints.
    %\item For other galaxies, radiative transfer models have successfully connected the observed infrared to submm radiation fields with independent models of stellar and dust physics.
    %\item This paper uses such a radiative transfer model to account for the the radiation field in the interstellar medium of the Milky Way between ultraviolet and submm wavelengths.
    %\item While previous studies had predicted the radiation field due to stars or the dust emission spectrum, this paper extends those by connecting the two with self-consistent radiative transfer calculations across a wide range of wavelengths.
    %\item While external galaxies are sometimes fairly close to edge-on, the Milky Way can only be observed through the disk, making modelling the radiation field more difficult due to the omnipresence of dust contamination.
    %\item The location of the sun in the Milky Way also means that there is a degeneracy between distance and luminosity of Milky Way stellar sources as observed from Earth, also making modelling the radiation field more difficult.
    %\item This paper assumes the galaxy is axially symmetric.  I think this effectively means they only model the radial dependence of the radiation field, and assume it does depend on distance perpendicular to the galactic disk.
    
%\end{itemize}

%Main thing from previous papers - gamma ray observations is sensitive to interstellar radiation field.  Need good modeling of interstellar radiation field to use gamma ray observations to use cosmic ray physics.  Easier to model observation from other galaxies than from the milky way because sun is off center in MW (introducing a degeneracy in distance between stars and luminosity).  Extragalactic observations, need face on to minimize dust obscuring the signal. \ca{This paragraph content is a relatively good concise set-up for that information.}

